The Tracking Tapered Gridded Estimator for the 21-cm power spectrum from MWA drift scan observations II: The Missing Frequency Channels

Missing frequency channels pose a problem for estimating $P(k_\perp,k_\parallel)$ the redshifted 21-cm power spectrum (PS) from radio-interferometric visibility data. This is particularly severe for the Murchison Widefield Array (MWA), which has a periodic pattern of missing channels that introduce spikes along $k_\parallel$. The Tracking Tapered Gridded Estimator (TTGE) overcomes this by first correlating the visibilities in the frequency domain to estimate the multi-frequency angular power spectrum (MAPS) $C_\ell(\Delta\nu)$ that has no missing frequency separation $\Delta\nu$. We perform a Fourier transform along $\Delta\nu$ to estimate $P(k_\perp,k_\parallel)$. Considering our earlier work, simulations demonstrate that the TTGE can estimate $P(k_\perp,k_\parallel)$ without any artifacts due to the missing channels. However, the spikes were still found to persist for the actual data, which is foreground-dominated. The current work presents a detailed investigation considering both simulations and actual data. We find that the spikes arise due to a combination of the missing channels and the strong spectral dependence of the foregrounds. Based on this, we propose and demonstrate a technique to mitigate the spikes. Applying this, we find the values of $P(k_\perp,k_\parallel)$ in the region $0.004 \leq k_\perp \leq 0.048\,{\rm Mpc^{-1}}$ and $k_\parallel > 0.35 \,{\rm Mpc^{-1}}$ to be consistent with zero within the expected statistical fluctuations. We obtain the $2\sigma$ upper limit of $\Delta_{\rm UL}^2(k)=(918.17)^2\,{\rm mK^2}$ at $k=0.404\,{\rm Mpc^{-1}}$ for the mean squared brightness temperature fluctuations of the $z=8.2$ epoch of reionization (EoR) 21-cm signal. This upper limit is from just $\sim 17$ minutes of observation for a single pointing direction. We expect tighter constraints when we combine all $162$ different pointing directions of the drift scan observation.

==> preamble.tex <==
% \makeatletter
% \newcommand{\ifmnras}[2]{\@ifclassloaded{mnras}{#1}{#2}}
% \makeatother
% \makeatletter
% \newcommand{\ifpasa}[2]{\@ifclassloaded{cup-journal}{#1}{#2}}
% \makeatother
% % % Font and Input
% \ifpasa{\usepackage[nopatch]{microtype}}{\usepackage{microtype}}
% \usepackage[T1]{fontenc}
% \ifpasa{}{\usepackage[utf8]{inputenc}}
% \usepackage{multicol}
% \ifpasa{}{\usepackage{newtxtext,newtxmath}}
% \usepackage{ae,aecompl}
% \usepackage{fix-cm}

% % % Linguistic
% \usepackage[english]{babel}
% \usepackage{csquotes}

% % % Layout
% \usepackage[svgnames]{xcolor}
% \definecolor{equationCol}{HTML}{D95F02}
% \definecolor{sectionCol}{HTML}{7570B3}
% \definecolor{citeCol}{HTML}{1B9E77}

% % \ifpasa{\usepackage{hyperref}}{\usepackage[colorlinks=true, linkcolor=sectionCol, citecolor=citeCol]{hyperref}}
% % \ifmnras{\usepackage{hyperref}}{\usepackage[colorlinks=true,linkcolor=blue, citecolor=blue, allcolors=blue]{hyperref}}

% \ifpasa{}{\ifmnras{}{\usepackage[a4paper, width=200mm, top=25mm, bottom=25mm]{geometry}}}

% \usepackage{fancyhdr}
% \pagestyle{fancy}
% \ifpasa{}{\usepackage{titlesec}}
% \ifpasa{}{\usepackage{cleveref}}

% \ifpasa{}{\crefformat{footnote}{#2\footnotemark[#1]#3}}

% % % Math
% \usepackage{mathtools}
% \usepackage{amsmath}
% \ifmnras{}{\usepackage{amssymb}}
% \usepackage{nicefrac}
% \ifpasa{}{\usepackage{breqn}}
% \usepackage{gensymb}

% % % % Tables
% % \usepackage{array}
% % \usepackage{booktabs}
% % \usepackage{arydshln}
% % \renewcommand{\arraystretch}{1.2}

% % % Graphics
% \usepackage{subcaption}
% % \usepackage{subfigure}
% \usepackage{graphicx}
% \usepackage{float}

% % % Science
% \usepackage{siunitx}

% % % Bibliography
% \ifpasa{}{\ifmnras{}{\usepackage[natbibapa, nodoi]{apacite}}}

% \ifpasa{}{\ifmnras{}{\usepackage{natbib}}}

% \usepackage{booktabs}
% \renewcommand{\arraystretch}{1.2}

% % The Astrophysical Journal -> ApJ
% \ifpasa{}{\ifmnras{}{\newcommand{\apj}{ApJ}}}

% % The Astronomical Journal -> AJ
% \ifpasa{}{\ifmnras{}{\newcommand{\aj}{AJ}}}

% % The Astrophysical Journal Letters -> ApJL
% \ifpasa{}{\ifmnras{}{\newcommand{\apjl}{ApJL}}}

% % Monthly Notices of the Royal Astronomical Society -> MNRAS
% \ifpasa{}{\ifmnras{}{\newcommand{\mnras}{MNRAS}}}

% % Publications of the Astronomical Society of the Pacific -> PASP
% \ifpasa{}{\ifmnras{}{\newcommand{\pasp}{PASP}}}

% % Nature -> Nature
% \ifpasa{}{\ifmnras{}{\newcommand{\nat}{Nature}}}

% %
% \ifpasa{}{\ifmnras{}{\newcommand{\aap}{AAP}}}

% %
% \ifpasa{}{\ifmnras{}{\newcommand{\prl}{Phys. Rev. Lett.}}}

% % % User Defined Functions

% % % Redefine eqref
% \newcommand*{\SavedEqref}{}
% \let\SavedEqref\eqref
% \renewcommand*{\eqref}[1]{%
%     \begingroup
%         \hyperseup{
%             linkcolor=equationCol,
%             linkbordercolor=equationCol,
%         }%
%         \SavedEqref{#1}%
%     \endgroup
% }

% % Column Vector
% \newcommand*\cvec[1]{\begin{bmatrix}#1\end{bmatrix}}

% % Line Break
% \newcommand*\lbreak{\\[\baselineskip]}

% %%%%%%%%%%%%% alias %%%%%%%%%%%%%
% \defcitealias{Chatterjee2024}{Paper~I}

